LSwarm: Efficient Collision Avoidance for Large Swarms with Coverage Constraints in Complex Urban Scenes

In this paper, we address the problem of collision avoidance for a swarm of UAVs used for continuous surveillance of an urban environment. Our method, LSwarm, efficiently avoids collisions with static obstacles, dynamic obstacles and other agents in 3-D urban environments while considering coverage constraints. LSwarm computes collision avoiding velocities that (i) maximize the conformity of an agent to an optimal path given by a global coverage strategy and (ii) ensure sufficient resolution of the coverage data collected by each agent. Our algorithm is formulated based on ORCA (Optimal Reciprocal Collision Avoidance) and is scalable with respect to the size of the swarm. We evaluate the coverage performance of LSwarm in realistic simulations of a swarm of quadrotors in complex urban models. In practice, our approach can compute collision avoiding velocities for a swarm composed of tens to hundreds of agents in a few milliseconds on dense urban scenes consisting of tens of buildings.

==> References.tex <==
\begin{thebibliography}{99}
\bibitem{c1} D. Alejo, J. A. Cobano, G. Heredia and A. Ollero, "Optimal Reciprocal Collision Avoidance with mobile and static obstacles for multi-UAV systems," 2014 International Conference on Unmanned Aircraft Systems (ICUAS), Orlando, FL, 2014, pp. 1259-1266.

%%
\bibitem{c2} Breitenmoser A., Martinoli A. (2016) On Combining Multi-robot Coverage and Reciprocal Collision Avoidance. In: Chong NY., Cho YJ. (eds) Distributed Autonomous Robotic Systems. Springer Tracts in Advanced Robotics, vol 112. Springer, Tokyo.

%%
\bibitem{c3} Choset H., Pignon P. (1998) Coverage Path Planning: The Boustrophedon Cellular Decomposition. In: Zelinsky A. (eds) Field and Service Robotics. Springer, London.

\bibitem{c4} S. Chung, A. A. Paranjape, P. Dames, S. Shen and V. Kumar, "A Survey on Aerial Swarm Robotics," in IEEE Transactions on Robotics, vol. 34, no. 4, pp. 837-855, Aug. 2018.

\bibitem{c5} P. Dames, M. Schwager, V. Kumar and D. Rus, "A decentralized control policy for adaptive information gathering in hazardous environments," 2012 IEEE 51st IEEE Conference on Decision and Control (CDC), Maui, HI, 2012, pp. 2807-2813.

%%
\bibitem{c6}de Lamadrid, J. G. (1994) "Avoidance of Obstacles With Unknown Trajectories: Locally Optimal Paths and Periodic Sensor Readings", The International Journal of Robotics Research, 13(6), pp. 496–507. 

%%
\bibitem{c7} Fiorini, P., \& Shiller, Z. (1998). "Motion Planning in Dynamic Environments Using Velocity Obstacles". The International Journal of Robotics Research, 17(7), 760–772.

\bibitem{c8} C. Fulgenzi, A. Spalanzani and C. Laugier, "Dynamic Obstacle Avoidance in uncertain environment combining PVOs and Occupancy Grid," Proceedings 2007 IEEE International Conference on Robotics and Automation, Roma, 2007, pp. 1610-1616.

%%
\bibitem{c9} Galceran, E., \& Carreras, M. (2013). "A survey on coverage path planning for robotics". Robotics and Autonomous Systems, 61, 1258-1276.

\bibitem{c10} M. Hamer, L. Widmer and R. D’andrea, "Fast Generation of Collision-Free Trajectories for Robot Swarms Using GPU Acceleration," in IEEE Access, vol. 7, pp. 6679-6690, 2019.

%%
\bibitem{c11} Hsu, D., Kindel, R., Latombe, J.-C., \& Rock, S. (2002). "Randomized Kinodynamic Motion Planning with Moving Obstacles". The International Journal of Robotics Research, 21(3), 233–255.

\bibitem{c12} W. Hönig, J. A. Preiss, T. K. S. Kumar, G. S. Sukhatme and N. Ayanian, "Trajectory Planning for Quadrotor Swarms," in IEEE Transactions on Robotics, vol. 34, no. 4, pp. 856-869, Aug. 2018.

%%
\bibitem{c13} Julian, B. J., Angermann, M., Schwager, M., \& Rus, D. (2012). "Distributed robotic sensor networks: An information-theoretic approach". The International Journal of Robotics Research, 31(10), 1134–1154.

\bibitem{c14} Chan Sze Kong, New Ai Peng and I. Rekleitis, "Distributed coverage with multi-robot system," Proceedings 2006 IEEE International Conference on Robotics and Automation, 2006. ICRA 2006., Orlando, FL, 2006, pp. 2423-2429.

%%
\bibitem{c15} B. O. Koopman. 1956. "The Theory of Search. II. Target Detection". Oper. Res. 4, 5 (October 1956), 503-531. DOI=http://dx.doi.org/10.1287/opre.4.5.503

%%
\bibitem{c16} Stefan Gottschalk M. C. L. Eric Larsen and D. Manocha. 1999. Proximity QueryPackage. (1999). http://gamma.cs.unc.edu/SSV/

\bibitem{c17} L. Martinez-Gomez and T. Fraichard, "Collision avoidance in dynamic environments: An ICS-based solution and its comparative evaluation," 2009 IEEE International Conference on Robotics and Automation, Kobe, 2009, pp. 100-105.

%%
\bibitem{c18} Mathewa, G., \& Mezic, I. (2010). "Metrics for ergodicity and design of ergodic dynamics for multi-agent systems".

\bibitem{c19} A. Ntawumenyikizaba, Hoang Huu Viet and TaeChoong Chung, "An online complete coverage algorithm for cleaning robots based on boustrophedon motions and A* search," 2012 8th International Conference on Information Science and Digital Content Technology (ICIDT2012), Jeju, 2012, pp. 401-405.

\bibitem{c20} I. Saha, R. Ramaithitima, V. Kumar, G. J. Pappas and S. A. Seshia, "Implan: Scalable Incremental Motion Planning for Multi-Robot Systems," 2016 ACM/IEEE 7th International Conference on Cyber-Physical Systems (ICCPS), Vienna, 2016, pp. 1-10.

%%
\bibitem{c21} Saska, M., Vonásek, V., Chudoba, J. et al. J Intell Robot Syst (2016) 84: 469. https://doi.org/10.1007/s10846-016-0338-z

\bibitem{c22} M. Schmittle et al., "OpenUAV: A UAV Testbed for the CPS and Robotics Community," 2018 ACM/IEEE 9th International Conference on Cyber-Physical Systems (ICCPS), Porto, 2018, pp. 130-139.

%%
\bibitem{c23} Schwager M., Dames P., Rus D., Kumar V. (2017) "A Multi-robot Control Policy for Information Gathering in the Presence of Unknown Hazards". In: Christensen H., Khatib O. (eds) Robotics Research. Springer Tracts in Advanced Robotics, vol 100. Springer, Cham

%%
\bibitem{c24} Spires S.V., Goldsmith S.Y. (1998) Exhaustive geographic search with mobile robots along space-filling curves. In: Drogoul A., Tambe M., Fukuda T. (eds) Collective Robotics. CRW 1998. Lecture Notes in Computer Science (Lecture Notes in Artificial Intelligence), vol 1456. Springer, Berlin, Heidelberg

%%
\bibitem{c25} Turpin, M., Michael, N., \& Kumar, V. (2014). "Capt: Concurrent assignment and planning of trajectories for multiple robots". The International Journal of Robotics Research, 33(1), 98–112.

%%
\bibitem{c26} van den Berg J., Guy S.J., Lin M., Manocha D. (2011) Reciprocal n-Body Collision Avoidance. In: Pradalier C., Siegwart R., Hirzinger G. (eds) Robotics Research. Springer Tracts in Advanced Robotics, vol 70. Springer, Berlin, Heidelberg

\bibitem{c27} J. van den Berg, Ming Lin and D. Manocha, "Reciprocal Velocity Obstacles for real-time multi-agent navigation," 2008 IEEE International Conference on Robotics and Automation, Pasadena, CA, 2008, pp. 1928-1935.

\bibitem{c28} J. van den Berg, J. Snape, S. J. Guy and D. Manocha, "Reciprocal collision avoidance with acceleration-velocity obstacles," 2011 IEEE International Conference on Robotics and Automation, Shanghai, 2011, pp. 3475-3482.

%%
\bibitem{c29} J. van der Berg, S. J. Guy, J. Snape, M. C. Lin, and D. Manocha. 2008. RVO2 Library:Reciprocal Collision Avoidance for Real-Time Multi-Agent Simulation.  (May2008). http://gamma.cs.unc.edu/RVO2/

\bibitem{c30} P. Velagapudi, K. Sycara and P. Scerri, "Decentralized prioritized planning in large multirobot teams," 2010 IEEE/RSJ International Conference on Intelligent Robots and Systems, Taipei, 2010, pp. 4603-4609.

%%
\bibitem{c31} Patrick Vincent and Izhak Rubin. 2004. A framework and analysis for cooperative search using UAV swarms. In Proceedings of the 2004 ACM symposium on Applied computing (SAC '04). ACM, New York, NY, USA, 79-86. DOI: https://doi.org/10.1145/967900.967919

\end{thebibliography}
